QuickSel: Quick Selectivity Learning with Mixture Models

Estimating the selectivity of a query is a key step in almost any cost-based query optimizer. Most of today's databases rely on histograms or samples that are periodically refreshed by re-scanning the data as the underlying data changes. Since frequent scans are costly, these statistics are often stale and lead to poor selectivity estimates. As an alternative to scans, query-driven histograms have been proposed, which refine the histograms based on the actual selectivities of the observed queries. Unfortunately, these approaches are either too costly to use in practice---i.e., require an exponential number of buckets---or quickly lose their advantage as they observe more queries. In this paper, we propose a selectivity learning framework, called QuickSel, which falls into the query-driven paradigm but does not use histograms. Instead, it builds an internal model of the underlying data, which can be refined significantly faster (e.g., only 1.9 milliseconds for 300 queries). This fast refinement allows QuickSel to continuously learn from each query and yield increasingly more accurate selectivity estimates over time. Unlike query-driven histograms, QuickSel relies on a mixture model and a new optimization algorithm for training its model. Our extensive experiments on two real-world datasets confirm that, given the same target accuracy, QuickSel is 34.0x-179.4x faster than state-of-the-art query-driven histograms, including ISOMER and STHoles. Further, given the same space budget, QuickSel is 26.8%-91.8% more accurate than periodically-updated histograms and samples, respectively.

==> additional_discussion.tex <==
\ignore{
\section{Join Selectivity \& Other Types}
\label{sec:prelim:join}

Query-driven selectivity estimation can be generalized in two orthogonal directions: (1) estimating the selectivity of a query including joins and (2) supporting more data types.

\ph{Selectivity for Join\texttt{+}Selection}
\cref{prob:sec} concerns the selectivity only for a single relation. However, the selectivity of a joined relation can also be computed by combining the selectivity estimates on a single relation and the selectivity of join conditions, under the assumption that the join conditions are independent of the selection predicates placed on individual tables~\cite{oracle_cbo}. For example, suppose that two predicates $P_1$ and $P_2$ are respectively placed on two relations $T_1$ and $T_2$, which are inner-joined on $T_1.C = T_2.C$.
Then, one heuristic rule for the inner-join selectivity is $s_{join} = 1 / \max(|\text{distinct}(T1.C)|, |\text{distinct}(T2.C)|)$~\cite{spark_cbo}. 
Let $s_1$ and $s_2$ be the selectivities of $P_1$ and $P_2$, respectively. Then, the number of the tuples of the joined relation can be computed as $|T_1| \cdot |T_2| \cdot s_{join} \cdot s_1 \cdot s_2$. This approach can also be applied to the other join selectivity rules~\cite{postgres_cbo,haas1996selectivity,van1993multiple}.


\ph{Other Data Types}
\cref{prob:sec} can be extended to support the relations containing discrete attribute values (e.g., integer, char) and the equality constraints on them, as follows. Without loss of generality, suppose that the domain of $C_i$ is $\{ 1, 2, \ldots, b_i \}$. Then, the constraint ``$C_i = k$'' is converted to the range constraint $k < C_i < k+1$; the domain of $C_i$ is converted to $(1, b_i + 1)$. Mathematically, this is equivalent to replacing a probability mass function with a probability density function consisting of \emph{dirac delta functions}.\footnote{A dirac delta function $\delta(x)$ outputs $\infty$ if $x = 0$ and outputs 0 otherwise while satisfying $\int \delta(x)\, dx = 1$.} Then, the summation of the original probability mass function can also be converted to the integration of the probability density function.
Moreover, the string data types (e.g., char, varchar) and the equality constraints on them can also be supported by internally maintaining a mapping from a string value to an integer and applying the technique described above for the integer data type.
}

\ignore{
\section{Warm Start}
\label{sec:training:warm}

One shortcoming of \method is that its accuracy can be low when the number of \emph{relevant} observed queries is small. This occurs in two cases: first, a relation was recently created, and not enough observed queries have been collected for the relation; second, the new workload significantly differs from the past workloads, rendering most past observed queries uninformative.

We can address this cold-start problem by incorporating existing static techniques (e.g., histograms~\cite{spark_cbo,sqlserver_cbo,ibm_cbo,oracle_online,gunopulos2005selectivity,ilyas2004cords,gunopulos2000approximating} or Most Common Values~\cite{postgres_cbo}) into query-driven selectivity estimation, as follows.

\ph{Histograms} The buckets constructed by any histogram construction algorithms, including equi-width, equi-depth, etc., can be expressed as observed queries in a straightforward way. For example, if 10\% tuples are included within the range (0,10), the range is a special case of a hyperrectangle (for a predicate) and the frequency is the selectivity. These information can then simply be incorporated in the observed query list of the query-driven selectivity estimation problem (\cref{prob:sec}).


\ph{Most Common Values} Most common values (MCVs) capture the frequency of high-frequency attribute values. For example, if a string value \texttt{'AAA'} appears in 2\% of the tuples (in a certain attribute), a pair (\texttt{'AAA'}, 0.02) is stored and used for selectivity estimation. Note that this is also a special case of an observed query. We already described how to handle the equality conditions in \cref{sec:prelim:join}.
}


\section{Relationship to Max Entropy}
\label{sec:disc:entropy}

The max-entropy query-driven histograms optimize their parameters (i.e., bucket frequencies) by searching for the parameter values that maximize the entropy of the distribution $f(x)$. We show that this approach is approximately equivalent to \method's optimization objective, i.e., minimizing MSE of $f(x)$ from a uniform distribution. The entropy of the probability density function is defined as $\minus \int f(x) \, \log( f(x) ) \, dx$. Thus, maximizing the entropy is equivalent to minimizing $\int f(x) \, \log( f(x) ) \, dx$, which is related to minimizing MSE as follows:
\begin{align*}
  \argmin \int f(x)\,  \log( f(x) ) \; dx 
  &\approx \argmin \int f(x)\, (f(x) - 1) \; dx \\
  &= \argmin \int (f(x))^2 \; dx
\end{align*}
since $\int f(x) \, dx = 1$ by definition. We used the first-order Taylor expansion to approximate $\log(x)$ with $x - 1$. Note that, when the constraint $\int f(x)\, dx = 1$ is considered, $f(x) = 1/|R_0|$ is the common solution to both the entropy maximization and minimizing MSE.


==> additional_exp.tex <==
\input{fig_tab/fig_exp_param}

\section{Additional Experiments: Impact of Data Correlation, Workload, and Parameter Count Control}
\label{sec:exp:param}
\barzan{prev subsection already talked about param count.
why r u flip flopping?}

We further studied how \method's accuracy is affected by data distribution, query workload distribution, and the number of its model parameters. 
\tofix{To control the number of model parameters, we manually controlled \method rather than using its default option (i.e., \# of model params = 4 $\times$ \# of observed queries).}

\ph{\tofix{Sensitivity to Data Correlation}}
To study how \method's accuracy changes based on different data \tofix{correlations}, we used \synthetic with different correlations. 
\tofix{In each case, \method trained its model using 100 observed queries; the error was measured using 100 different queries.}
\barzan{u say to study diff dists we used this one dist w diff params!!!}
As shown in \cref{fig:exp:param:a}, 
    the errors were almost identical \tofix{for all cases with different correlations.}
    % except when
    % the correlation was considerably higher 
    % (i.e., $\geq$0.9). 
    
    % This is because, when the correlation is high, 
    %     only a small number of assertions are actually useful \tofix{(i.e., the probability distribution is almost zero for most areas)}, 
    %     \yongjoo{Make a connection here.}
    %     which leads to slightly lower accuracy. 
    %     Nevertheless, \method still produced highly accurate estimates even under high correlations (i.e., less than 0.5\% error).



\ph{Workload Shifts}
We also studied  \method's accuracy 
under situations where the 
query workload shifts over time. 
Here, we generated the  \synthetic dataset
with
% data points using a bivariate normal with mean (0.5, 0.5) and 
correlation 0.5.
We generated  queries with different predicates,
    with each predicate being a different rectangle in the 2-dimensional 
    space.\footnote{\tofix{The purpose of this synthetic dataset is to 
        simulate a workload shift, we study high-dimensional data and queries in \cref{fig:exp:param:d}.}}
We simulated three scenarios of workload shifts
    by modifying these rectangular predicates. 
First, we created a \emph{random-shift} workload by choosing random rectangles in the space. We also created a \emph{sliding-shift} workload by gradually moving the rectangles from the left-tail of the normal
        distribution towards the right-tail.
Third, we created a \emph{no-shift} workload by using the same rectangle for all queries.

 %To catest \method's accuracy, this experiment used a slightly different approach.
In each scenario, we first trained \method on the first 10 observed queries (i.e., sequence numbers: 1--10) and   measured the accuracy on the next 10 observed queries (i.e., sequence numbers: 11--20). 
Then, we trained \method on the first 20 observed queries (i.e., sequence numbers: 1--20) and measured the accuracy using the next 10 observed queries (i.e., their sequence numbers: 21--30). We kept increasing the number of observed queries until we reached 
    1,000 observed queries for training.
The results are plotted in \cref{fig:exp:param:b}. 

\barzan{this para should change} \yongjoo{Changed}
\tofix{As expected, the errors were highest for random shift workload. However, the error gradually decreased as \method observed more queries; when 100 queries were observed, the relative error was only 1.2\% for the random shift workload. The errors were lower in general for other workloads.}

% \tofix{Initially, the errors were lower for the shifting workload, which was only because the queries around the bottom-left corner were associated with low selectivities (thus, lower absolute errors). However, the errors for the static workload decreased quickly. In contrast, the errors for the shifting workloads elevated slightly. Nevertheless, the errors were low in general (i.e., less than 0.5\%). The primary reason \method yielded low errors, even for the \emph{new} areas, was that \method exploited the global property of every probability distribution. That is, the probability distribution function must sum (or integrate) to one, which is reflected in \method's optimization constraint; thus, learning the probability distribution of one area also refines the probability distribution estimates for the other areas, even though the other areas are never queried.}


\ph{Model Parameter Count}
Third, we studied the relationship between the number of model parameters and \method's accuracy, \tofix{with a fixed number of observed queries: 100}. 
% Recall that the 
% number of \method's parameters can be         controlled by 
%     choosing the number of centers in its $k$-means clustering (\cref{sec:model:sub}).
% Here, we used 100 queries for training; 
The dataset 
was \synthetic with correlation 0.5.
\cref{fig:exp:param:c} shows the results. 
As expected, the errors were relatively higher when the number of model parameters was extremely small (i.e., 10). 
However, as soon as the number of model parameters reached 50 the error
    was drastically reduced.


\ph{Column Set Size}
\tofix{
Lastly, we studied the relationship between the \emph{column set size} and the error of \method; \method approximates the join distribution of the column set.
For this experiment, we generated the datasets from multivariate normal distributions; for each dataset, we generated queries with the same average selectivities and used them for both training and tests.

\cref{fig:exp:param:c} shows the result. For comparison, we also report the error of AutoSample, which is not sensitive to the data dimension by nature. In the figure, \method was more accurate than AutoSample when the column set size was less than 8 while the error of \method was larger than AutoSample for bigger column sets.

Note that this property of \method does not reduce its practical usefulness
since the selectivity of a big column set can be estimated by the selectivities of smaller columns sets that partitions the big column set~\cite{oracle_cbo,postgres_cbo}.
}
    

==> backup.tex <==
\subsection{LCE Architecture}
\label{sec:overview:archi}

This section describes the architecture of the database system with a LCE module. Let $S$ be the LCE module. Also, let $(s_i, b_i)$ be a pair of the $i$-th selection predicate and the number of the data items that satisfy the $i$-th selection predicate. We call such a pair a \emph{cardinality assertion}. There are many kinds of selection predicates, depending on attribute types (e.g., \texttt{date}, \texttt{decimal}, etc.) or for mere convenience (e.g., \texttt{in}, \texttt{between}, etc.); however, many predicates (e.g., equality on discrete attributes) can be converted to range constraints on real values (e.g., by mapping discrete attribute values to integers). In this work, our discussion focuses on such ranges constraints. Note that our work is not applicable to the predicates that cannot be converted to range constraints, e.g., textual filters.

% There are some special cases that ask for more attention. For example, \texttt{shipdate = '2017-1-1'} should be internally translated into \texttt{shipdate >= '2017-01-01 00:00:00AM' and shipdate <= '2017-01-31 23:59:59PM'}. Also, equality constraints on discrete attributes should be converted to range constraints on corresponding integer mappings: for example, \texttt{shipmode = 'AIR'} to \texttt{shipmode >= 0 and shipmode < 1}, where \texttt{'AIR'} is mapped to the integer 0. However, these types of conversions can be handled easily in practice, so this does not limit the generality of our work.

The goal of $S$ is, given $n$ cardinality assertions, namely $(s_1, b_1),\allowbreak \ldots, \allowbreak (s_n, b_n)$, estimate $b_{n+1}$ for $s_{n+1}$. After estimating $b_{n+1}$, $S$ is provided the actual value of $b_{n+1}$; thus, it can compose a new density assertion for $(n+1)$-th query. This process continues for $b_{n+2}$, $b_{n+3}$, and so on.

\input{fig_tab/fig_architecture}

\Cref{fig:archi} depicts how $S$ works with a database system's query optimizer and query executor. Whenever the query optimizer receives a query, it consults $S$ to obtain a cardinality estimate for the query. Then, the query optimizer chooses an optimal query plan based on the cardinality estimate provided by $S$. The database system's query executor processes the query using the optimal query plan. After processing the query, the database system knows the actual number of the data items that satisfy the selection predicate of the query. This information is provided to $S$ in the form of cardinality assertion. As the database system processes more queries, $S$ collects more cardinality assertions, so $S$'s cardinality estimates become more accurate.

In reality, a single query might need multiple cardinality estimates: for example, the query involves multiple tables. In this case, $S$ treats those cardinality estimates separately. This situation does not alter the general workflow of $S$.

% Note: this section does not need to define any notations or attributes. Only define $N$, the total number of tuples in a table, and $n$, the number of past queries. Does not discuss join; focus on a single table (maybe i can mention that we can treat a joined table as a single table).

\input{fig_tab/tab_previous_work}

\subsection{Benefits and Limitations of LCE}
\label{sec:overview:benefit}
\label{sec:overview:limit}

\ph{Benefits}
In comparison to offline-computed cardinality estimation techniques, such as histograms and sampling-based methods, LCE methods have the following benefits.
\begin{enumerate}
\item \textbf{Low offline costs}: LCE does not require upfront offline computation time for scanning a database; cardinality assertions are low-overhead byproducts of query processing. One might prefer LCE methods to optionally perform some amount of offline computations to prevent a cold-start problem (\cref{sec:method:per}); however, its cost is still not larger than the costs for constructing simple histograms.
\item \textbf{Able to capture correlations among attributes}: In general, LCE methods do not assume any independence among different attributes, which is also true for \method. Note that simple per-attribute histograms make the strong independence assumptions among different attributes; thus, they are fundamentally unable to capture correlations, which are frequently present in real datasets. Although multidimensional histograms are able to capture those correlations, their space complexity is an exponential function of the number of columns; thus, the multidimensional histograms are impractical if the number of columns is more than a few.
\item \textbf{High accuracy even for sparse areas}: The cardinality assertions for spare areas are as accurate as the cardinality assertions for dense areas, because they are composed exact number of the data items that satisfy their respective selection predicates. On the other hand, sampling-based techniques are effective only for relatively dense areas; for sparse areas, a random sample may not include any data items for sparse areas, in which case, they will provide poor quality cardinality estimates.
\end{enumerate}
\Cref{tab:comp} summarizes these benefits of LCE with computational complexity analysis of each approach. These benefits make LCE methods useful for handling ad-hoc analytic queries.


\ph{Limitations}
LCE refines its estimation quality based on past query answers. As a result, the system with a LCE method has the following limitations:
\begin{enumerate}
\item \textbf{Cold-start}: The system with a LCE method initially has zero cardinality assertions. In this case, the system is unable to provide any estimates.
\item \textbf{Cold-area}: The system with a LCE method incrementally refines its knowledge on the underlying probability distribution, and this refinement is possible for queried ranges. As a result, the system is less effective for the ranges that have not been queried in the past.
\end{enumerate}
\method addresses these issues by incorporating a pre-built histogram (see \cref{sec:method:per}).


\subsection{Join Cardinality Estimation}
\label{sec:overview:join}



==> discussion.tex <==
%!TEX root = main.tex

\section{Properties of Crumbs}
\label{sec:disc}

This section provides two technical discussions. First, \cref{sec:disc:consistency} shows why \system can construct a probability distribution that well approximates the true probability distribution. Second, \cref{sec:disc:entropy} presents that the probability distribution obtained by \system is closely related to the maximum entropy distribution, which is the distribution that can be obtained by assuming nothing but provided.


\subsection{Increasing Consistency with More Queries}
\label{sec:disc:consistency}




% \subsection{Optimal Kernel-based PDF}
% \label{sec:disc:consistency}

% \tofix{Think about what is the optimal weights of kernels.}

% Why looser consistency OK?
% larger number of constraints help more.
% we anyway need to relax the constraints for updatable data.


% Maybe this should not be a separate subsection. Let's think about it more later.


==> failure.tex <==
\section{Limitations of Histogram}
\label{sec:fail}

Previous LCE work represents a data distribution using a histogram-like structure; that is, the domain of attributes is partitioned into disjoint regions, and the weights are assigned for those regions. The assigned weights are consistent with the given cardinality assertions, namely, $(s_1, b_1), \allowbreak \ldots, \allowbreak (s_n, b_n)$. For constructing this histogram-like structure, workload-sensitive partitioning must precede.

In this section, we overview the partitioning method used by previous LCE methods and analyze its complexity. In addition, we discuss the hardness of workload-sensitive partitioning by providing several our attempts.


\subsection{Workload-Sensitive Partitioning}
\label{sec:fail:partition}

We discuss ISOMER's partitioning algorithm~\cite{srivastava2006isomer}, which is a variant of STHoles~\cite{}.

\input{fig_tab/fig_isomer_partition}

Previous work defines histogram bins through partitioning spaces. In this way, it is guaranteed that bins are disjoint regions, and a collections of those bins cover the entire space.

\Cref{fig:isomer_partition}

Mention that the masses of bins are assigned so that they are consistent with the past query answers. Describe this using matrix and vectors. $A$: the queries and their inclusion of bins, $x$: the mass assignments to the bins (all non-negative), $b$: the past query answers.



\subsection{Exponential Number of Partitions}
\label{sec:fail:exp}

\input{fig_tab/fig_isomer_count_regions}

The main problem of the previous work, ISOMER, is its expensive computational cost. Specifically, it has two issues:
\begin{enumerate}
    \item The number of regions grows as $O(n^2)$. Our simple experiment shows that the number of regions is over 1,000 only for 40 queries.
    \item It finds the density of each region, but the number of region it can handle is only a few hundreds.
\end{enumerate}

\isomer addresses this by keeping a very small number of past queries; as a result, \isomer is unable to use most of past query answers.



\subsection{Other Workload-sensitive Partitioning}
\label{sec:voronoi}

Works well for high-dimensional data

\input{fig_tab/fig_work_sensitive_bins}

Two trials:
\begin{enumerate}
\item partition selection ranges
\item partition in high-dimensional space
\end{enumerate}



Voronoi diagram

I would like to discuss why partition-based techniques are hard.




% \subsection{Optimal Bin Weights}
% \label{sec:fail:opt}

% Define histograms. Make a relation to probability distribution function.



==> fig_tab/fig_exp_performance_impact.tex <==
\begin{figure*}[t]
\label{fig:exp:impact}

\pgfplotsset{impactfig/.style={
    width=70mm,
    height=35mm,
    xmin=0,
    xmax=1000,
    ymin=0,
    ymax=8000,
    xlabel=Number of Observed Queries,
    ylabel=Query Latency,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    xtick={0, 100, ..., 1000},
    % xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
    ytick={0, 2000, ..., 8000},
    yticklabels={0 sec, 2 sec, 4 sec, 6 sec, 8 sec},
    scaled y ticks = false,
    % yticklabels={0\%, 10\%, 20\%, 30\%},
    % xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
    % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    ylabel shift=-2pt,
    xlabel shift=-2pt,
    legend style={
        at={(0, 1.1)},anchor=south west,column sep=2pt,
        draw=black,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=10pt}
    },
    legend cell align={left},
    legend columns=4,
    every axis/.append style={font=\footnotesize},
    ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
}}

% \centering

\begin{subfigure}[b]{0.48\linewidth}
% \centering
\hspace*{6mm}
\begin{tikzpicture}
\begin{axis}[impactfig]
    
\addplot[mark=*,mark size=1.5,mark options={fill=vintageblack,draw=vintageblack},
thick,draw=vintageblack,
]
table[x=x,y=y] {
x y
0 4155
50 4084
100 4326
150 4015
200 3801
250 4177
300 4197
350 4453
400 4864
450 4263
500 3679
550 4008
600 4185
650 4504
700 3864
750 4384
800 3990
850 4516
900 4939
950 4839
1000 4142
};

\addplot[mark=triangle*,mark size=2,mark options={fill=vintagegreen,draw=vintagegreen},
thick,draw=vintagegreen,
]
table[x=x,y=y] {
x y
0    4806
50   4828
100  4965
150  5467
200  4125
250  4517
300  4288
350  4540
400  4968
450  4376
500  3945
550  5556
600  4164
650  5128
700  3944
750  4458
800  4069
850  4736
900  5116
950  4996
1000 4480
};

\addplot[mark=*,mark size=1.5,mark options={fill=vintageorange,draw=vintageorange},
thick,draw=vintageorange,
]
table[x=x,y=y] {
x y
0    4412
50   4935
100  4631
150  4215
200  4046
250  4472
300  4281
350  4610
400  5000
450  4382
500  3947
550  5367
600  4280
650  5290
700  3964
750  4442
800  4032
850  4590
900  4904
950  5054
1000 4199
};

\addlegendentry{Postgres Default}
\addlegendentry{Postgres with AutoSample}
\addlegendentry{Postgres with \method}


\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{Filters on Uncorrelated Columns}
\label{fig:exp:impact:a}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\linewidth}
% \centering
\begin{tikzpicture}
\begin{axis}[impactfig]
    
\addplot[mark=*,mark size=1.5,mark options={fill=vintageblack,draw=vintageblack},
thick,draw=vintageblack,
]
table[x=x,y=y] {
x y
0    6806
50   6613
100  6868
150  6709
200  6801
250  6698
300  6762
350  6520
400  6988
450  7095
500  6875
550  6992
600  6805
650  6964
700  6871
750  6692
800  6845
850  7018
900  6835
950  6721
1000 6978
};

\addplot[mark=triangle*,mark size=2,mark options={fill=vintagegreen,draw=vintagegreen},
thick,draw=vintagegreen,
]
table[x=x,y=y] {
x y
0	6729
50	6613
100	6858
150	6695
200	6804
250	6697
300	6762
350	6513
400	6973
450	7093
500	6859
550	6976
600	6799
650	6958
700	6880
750	6689
800	6847
850	7021
900	6826
950	6714
1000	6962
};

\addplot[mark=*,mark size=1.5,mark options={fill=vintageorange,draw=vintageorange},
thick,draw=vintageorange,
]
table[x=x,y=y] {
x y
0	6642
50	4952
100	4615
150	4088
200	3911
250	4369
300	4367
350	3936
400	3974
450	4084
500	4170
550	4419
600	4693
650	3858
700	3091
750	4106
800	3751
850	4184
900	3131
950	2923
1000	3227
};

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{Filters on Uncorrelated Columns}
\label{fig:exp:impact:b}
\end{subfigure}


\caption{
\revision{C3}{Impact on join query performance.
We compared
(1) Postgres default, (2) Postgres with AutoSample, and 
(3) Postgres with \method. Left: When filters were on uncorrelated columns, no significant difference observed. Right: When filters were on correlated columns, Postgres with \method showed significant performance gains; 42\% average  and 56\% max improvement compared to Postgres default after observing 100 or more queries. }}
\end{figure*}


==> fig_tab/fig_kernels.tex <==
\begin{figure}[h]
    \centering
    
    \caption{Probability density function expressed in terms of kernels (weighted hyper-rectangles).}
    \label{fig:kernels}
\end{figure}

==> fig_tab/fig_work_sensitive_bins.tex <==
\begin{figure}[h]
    \centering
    
    \caption{Difficulties in creating workload-sensitive bins.}
    \label{fig:work_sensitive_bins}
\end{figure}

==> fig_tab/tab_previous_work.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l c c c c r}
\hline
\multirow{2}{*}{Approach}  &  Able to capture  &  Workload  &
    Accurate for & \multirow{2}{*}{Scalable}  & Estimation\\
    & correlation & adaptive & sparse areas & & time complexity\\ \hline
Per-attribute histogram    & & & & \checkmark & $O(b \cdot d)$ \\
Multidimensional histogram & \checkmark & & & & $O(b^d)$ \\
Sample-based estimation    & \checkmark & & & \checkmark & $O(m)$ \\
Previous selectivity learning method \cite{srivastava2006isomer,??} & \checkmark &
    \checkmark & \checkmark & & $O(2^n)$ \\
\textbf{Our selectivity learning method (\method)}  & \checkmark &
    \checkmark & \checkmark & \checkmark & $O(n)$ \\ \hline
\end{tabular}
\caption{Comparison of density estimation methods. For histograms, $b$ is the number of histogram bins for each attribute. For sampling-based estimation, $m$ is the number of sampled tuples. For LDE methods, $n$ is the number of past selection predicates.}
\label{tab:comp}
\end{table*}

==> fig_tab/tab_sl_class.tex <==
\begin{table}[t]
\caption{Approaches to refining selectivity estimates}
\label{tab:sl:class}

\centering
\small
% \def\arraystretch{1.5}
\begin{tabular}{p{25mm} c c c}
\toprule
\textbf{Approach}
  & \begin{tabular}{@{}c@{}}\textbf{Exp.~Bucket} \\ \textbf{Counts}\end{tabular}
  & \begin{tabular}{@{}c@{}}\textbf{Fast} \\ \textbf{Training}\end{tabular}
  & \begin{tabular}{@{}c@{}}\textbf{High} \\ \textbf{Accuracy}\end{tabular} \\
\midrule
% \begin{tabular}{@{}l@{}}Freq-split \\ histograms\end{tabular}
Freq-split Histograms
  & No & Yes & No \\[5pt]
% \begin{tabular}{@{}l@{}}MaxEnt \\ histograms\end{tabular}
MaxEnt Histograms
  & Yes & No & Yes \\[5pt]
% \begin{tabular}{@{}l@{}}Mixture \\ Model\end{tabular}
Mixture Model
  & No & Yes & Yes \\
\bottomrule
\end{tabular}

\end{table}

==> fig_tab/tab_speedup.tex <==
\begin{table}[t]
\caption{Training Time for 1\% Error}
\centering
\small
\begin{tabular}{l r r r}
\toprule
Dataset & ISOMER (sec) & \method (sec) & \textbf{Speedup} \\
\midrule
\dmv    & 3491.321 & 1.784   & 1,957$\times$ \\
\insta  & 18.318   & 0.001   & 18,318$\times$ \\
\bottomrule
\end{tabular}
\end{table}

==> proofs.tex <==
% \vspace{-10mm}

\section{Proof}
\label{sec:proofs}


\begin{proof}[Proof to \cref{thm:quadratic}]
The theorem can be shown by substituting the definition of \method's model (\cref{eq:mm}) into the probability density function $f(x)$ in \cref{eq:prob:density}.
Note that minimizing $(f(x) - g_0(x))^2$ is equivalent to minimizing $f(x) \, (f(x) - 2 \, g_0(x))$, which is also equivalent to minimizing $(f(x))^2$ since $g_0(x)$ is constant over $B_0$ and $\int f(x) \, dx = 1$.

The integration of $(f(x))^2$ over $B_0$ can be converted to a matrix multiplication, as shown below:
\begin{align*}
\int (f(x))^2  \; dx 
% = \int (f(x))^2 - \frac{2 f(x)}{|R_0|}\; dx
  &= \int \left[ \sum_{z=1}^m \frac{w_z \, I(x \in G_z)}{|G_z|}  \right]^2 
    % - \sum_{z=1}^m \frac{2 \, w_z \, I(x \in G_z)}{|G_z| \, |R_0|} 
  \; dx \\
  &= \int \sum_{i=1}^m \sum_{j=1}^m \frac{w_i w_j}{|G_i| |G_j|} \,
      I(x \in G_i) \, I(x \in G_j) \; dx \\
    % &\quad - \int \sum_{z=1}^m \frac{2 \, w_z \, I(x \in G_z)}{|G_z| \, |R_0|}
    %   \; dx \\
  &= \sum_{i=1}^m \sum_{j=1}^m \frac{w_i \, w_j}{|G_i| \, |G_j|}
     \int I(x \in G_i \land x \in G_j) \; dx \\
    % &\quad - \sum_{z=1}^m \frac{2 \, w_z}{|G_z| \, |R_0|} \int I(x \in G_z) \; dx \\
  &= \sum_{i=1}^m \sum_{j=1}^m \frac{w_i w_j}{|G_i| |G_j|} \, |G_i \cap G_j|  \\
    % - \sum_{z=1}^m \frac{2\, w_z}{|R_0|} \\
  &= \begin{bmatrix}
       w_1 \\
       w_2 \\
       \vdots \\
       w_m
     \end{bmatrix}^\top
     %
     \begin{bmatrix}
       \frac{|G_1 \cap G_1|}{|G_1| |G_1|}  & \cdots & \frac{|G_1 \cap G_m|}{|G_1| |G_m|} \\
       \vdots & & \vdots \\
       \frac{|G_m \cap G_1|}{|G_m| |G_1|}  & \cdots & \frac{|G_m \cap G_m|}{|G_m| |G_m|}
     \end{bmatrix}
     %
     \begin{bmatrix}
       w_1 \\
       w_2 \\
       \vdots \\
       w_m
     \end{bmatrix} \\
  &= \ww^\top Q \, \ww
\end{align*}

Second, we express the equality constraints in an alternative form. Note that the left-hand side of each equality constraint, i.e., $\int_{B_i} f(x) \, dx$, can be expressed as:
\begin{align*}
&\int_{B_i} f(x) \; dx 
= \int_{B_i} \, \sum_{j=1}^m \, \frac{w_j}{|G_j|} \, I(x \in G_j) \; dx \\
&= \sum_{j=1}^m \, \frac{w_j}{|G_j|} \, \int_{B_i} I(x \in G_j) \; dx \\
&= \sum_{j=1}^m \, \frac{w_j}{|G_j|} \, |B_i \cap R_j| \\
&= \begin{bmatrix}
       \frac{|B_i \cap G_1|}{|G_1|} &
       \cdots &
       \frac{|B_i \cap G_m|}{|G_m|}
   \end{bmatrix}
   \begin{bmatrix}
       w_1 \\
       \vdots \\
       w_m
   \end{bmatrix}
\end{align*}
Then, the equality constraints, i.e., $\int_{B_i} f(x) \, dx = s_i$ for $i = 1, \ldots, n$, can be expressed as follows:
\begin{align*}
&\begin{bmatrix}
       \frac{|B_1 \cap G_1|}{|G_1|} &
       \cdots &
       \frac{|B_1 \cap G_m|}{|G_m|} \\
       \vdots & \ddots & \vdots \\
       \frac{|B_n \cap G_1|}{|G_1|} &
       \cdots &
       \frac{|B_n \cap G_m|}{|G_m|}
   \end{bmatrix}
   \begin{bmatrix}
       w_1 \\
       \vdots \\
       w_m
   \end{bmatrix}
   = 
   \begin{bmatrix}
       s_1 \\
       \vdots \\
       s_m
   \end{bmatrix} \\
&\Rightarrow \quad A \ww = \ss
\end{align*}

Finally, $\ww^\top \bm{1} = 1$ if and only if $\int f(x) = 1$, and $\ww \succcurlyeq \bm{0}$ for arbitrary $G_z$ if and only if $\int f(x) \ge 0$.
\end{proof}

==> space.tex <==
\section{Crumb Extension}
\label{sec:space}







\subsection{Extending Data Types}

The description in \cref{sec:method} focused on the relation that consists of only real-valued attributes. We briefly describe how to extend the core idea to other data types: integer and string.




ISOMER reduces the histogram size by discarding ``unimportant'' QFRs.
